Gecko: Versatile Text Embeddings Distilled from Large Language Models

We present Gecko, a compact and versatile text embedding model. Gecko achieves strong retrieval performance by leveraging a key idea: distilling knowledge from large language models (LLMs) into a retriever. Our two-step distillation process begins with generating diverse, synthetic paired data using an LLM. Next, we further refine the data quality by retrieving a set of candidate passages for each query, and relabeling the positive and hard negative passages using the same LLM. The effectiveness of our approach is demonstrated by the compactness of the Gecko. On the Massive Text Embedding Benchmark (MTEB), Gecko with 256 embedding dimensions outperforms all existing entries with 768 embedding size. Gecko with 768 embedding dimensions achieves an average score of 66.31, competing with 7x larger models and 5x higher dimensional embeddings.

==> defns.tex <==
%
% A useful set of commands
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{bbm}

\usepackage{algorithm}
\usepackage{algorithmicx}

\usepackage[most]{tcolorbox}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{changepage}
\usepackage{enumitem}

\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}


\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}



\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

% For bold vector symbols
\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}

\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vupsilon}{\myvecsym{\upsilon}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vxn}{\vx^{(n)}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mbox{const}}
\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}

\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\st}{\mbox{  s.t.  }}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}

\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathrm{KL}\left[{#1}\|{#2}\right]}
\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
%\newcommand{\E}{E}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
%\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expect}[2]{\mathds{E}_{{#1}} \left[ {#2} \right]}
\newcommand{\expectGiven}[3]{\mathds{E}_{{#1}} \left[ {#2} \mid {#3} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\VarGiven}[3]{\mbox{Var}_{{#1}}\left[ {#2} \mid {#3}\right]}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
%\newcommand{\mode}[1]{\mbox{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}



\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\supp}{\mbox{supp}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}


%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}


\newcommand{\condSet}{\mathcal{S}}
\newcommand{\condSetC}{\mathcal{\lnot S}}




==> sections/dataset.tex <==
\section{Dataset}
% For training \ours{}, we first generate \dataset{} using LLMs.
% We introduces how we generate a diverse set of queries and decide which passages to use as positive or negative targets.

In this section, we introduce our two-stage approach that uses LLMs to generate \dataset{}, the \textbf{F}ew-shot Prompted \textbf{Ret}rieval dataset (\cref{sec:fret}).
Then, we explain how we extend this dataset to add classification, which typically requires different techniques in order to make the contrastive learning work within a single compact model (\cref{sec:data_classificaiton}).
Finally, we describe additional datasets for the pre-finetuning and fine-tuning stages (\cref{sec:data_additional}), which we seamlessly combine with \dataset{} through standardized formatting.

%Then we describes how we incorporate classification datasets into the contrastive learning framework. Finally, we describes the additional training and finetuning datasets used for pushing the limit of \ours{}.

% \jinhyuk{more intro}

\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\columnwidth]{figures/fret-overview}
	\caption{Overview of \dataset{}.
	Given a sampled passage from the Web, \dataset{} first utilizes LLMs to generate a relevant task and a query for the passage (top).
	Each query and task is fed into a pre-trained retriever to mine both positive and negative passages where another LLM decides which passage to use as positive or negative (bottom).
	\jinhyuk{change examples + bigger font}}
	\label{fig:fret_overview}
\end{figure}

\subsection{\dataset{}: Two-Step LLM Distillation}\label{sec:fret}
% \jinhyuk{mention license issue?}
% \jinhyuk{dataset size table}

Traditional approaches to training embedding models often rely on large, manually labeled datasets. However, creating such datasets is time-consuming, expensive, and can introduce undesirable biases.
% While such datasets are valuable, they may not be reusable if the definition of the task or the underlying corpus changes.
In this work, we present a novel method for generating synthetic data for training multi-task text embedding models, leveraging the power of LLMs through a two-step distillation process.
The overall process of generating \dataset{} is illustrated in \Cref{fig:fret_overview}.

\paragraph{LLM-based Diverse Query Generation}
% One of the key challenges in training a versatile embedding model is the need for a large amount of high-quality queries.
One of the challenges of using manually crafted queries is to ensure that the queries cover a diverse set of tasks and linguistic patterns.
With LLMs, these variables are relatively easier to control as we can design the prompt to specify the diversity.
% This process fosters a more robust and versatile retrieval system.
In this work, we employ few-shot prompts to control the diversity of queries.
Our LLM is instructed to read a sampled Web passage and generate both the task description and a relevant query that the passage can answer:
\begin{equation*}
   \text{LLM}(\mathbb{P}_\text{QG},  p_\text{seed}) \rightarrow (t, q)
\end{equation*}
where $p_\text{seed}$ is a passage drawn randomly from the Web corpus $\mathcal{C}$ and $\mathbb{P}_\text{QG}$ is a fixed prompt with query generation examples.
The prompt, $\mathbb{P}_\text{QG}$, is fixed for every example and consists of few-shot examples and instructions.  
The LLM generates a task description $t$, which describes the type of retrieval such as \textit{`Given a query, find a passage that has the answer to the query'} (question answering) or \textit{`Given a query, find a passage that allows you to check whether the query is true or not'} (fact checking), and also a query $q$ that follows such task.
By sampling the task description, we guide the LLM to produce a wide range of queries.
These pairs are later used to train our embedding models so that they can make the model follow various instructions.
% \inaim{It may be good to explain what is the label here.}

Each input passage $p_\text{seed}$ is drawn from a large Web corpus.
The Web corpus inherently contains diverse topics and styles, which also act as a source of the diversity of generated queries.
Generating the task string also offers some control over generation diversity, as the tasks in the prompt can be modified to suit the downstream application.
Note that, in principle, our method can be applied to any corpus similar to \citet{dai2022promptagator}, but our method is different from approaches such as~\citet{wang2023improving} where LLMs generate both queries and passages.
\mjb{There is some duplication in the points expressed in the above section (diversity is from task, as well as from web corpus). Would be good to dedup and also reorder to a more problem/solution presentation.}

\paragraph{LLM-based Positive and Negative Mining}
Most models that utilize synthetic queries are trained with $(q, p_\text{seed})$ pairs assuming that $p_\text{seed}$ is a good positive target for $q$~\citep{dai2022promptagator,jeronymo2023inpars}.
% However, this approach limits the model performance due to its focus on local relevance.
While this is partly true for most cases, we hypothesize that, from the large Web, there could be a more relevant passage than $p_\text{seed}$.
Essentially, we have sampled $\operatorname{P}(q \mid p_\text{seed})$, but this is no guarantee that $\operatorname{P}(p_\text{seed} \mid q)$ is large.
This intuition is supported by our observation that generated queries often focus on a particular aspect of a relatively long passage.
% LLM has not seen every passage in the corpus and we do not know if the query that it generates actually distinguishes this passage from any other, or even if this passage is the best passage for the generated query.
Hence, we propose a method that leverages LLMs to discover more relevant positive passages along with a good hard negative for the generated query.
% by re-examining the global context.

In particular, we use an existing embedding model\footnote{In this work, we train an initial embedding model with $(q, p_\text{seed})$ pairs with in-batch random negatives.} to retrieve top $N$ neighbors $P=[p^{(1)}, \dots, p^{(N)}]$ from the corpus given a generated query $q$.
We then employ the same LLM used for the query generation to rank these retrieved passages based on their relevance to the query. 
%We introduce a simple method that combines  multiple few-shot prompted LLM to enhance relevance ranking. 
Specifically, we use two well-known few-shot prompted LLM ranking functions: query likelihood and relevance classification.
Query likelihood~\citep{Sachanql} uses an LLM to measure the log-likelihood of a generated query $q$ given a passage $p_i$, i.e., $\text{QL}(q, p_i)=\text{LLM}(q|p_i, \mathbb{P}_\text{QL})$, where $\mathbb{P}_\text{QL}$ is a prompt containing selected few-shot examples for query likelihood~\citep{drozdov2023parade}.
% (i.e. pairs of a relevant passage and a query).
Relevance classification~\citep{zhuang2023beyond} uses an LLM to measure the log-likelihood of a specific relevance label given the query $q$ and a passage $p_i$, i.e., $\text{RC}(q, p_i)=\text{LLM}(\text{label}|q, p_i, \mathbb{P}_\text{RC})$, where $\mathbb{P}_\text{RC}$ is a prompt with few-shot examples for grading the relevance of each query-passage pair.
Our pilot study demonstrated that each prompting method (i.e. QL and RC) excels in different tasks, so we ensemble the rankings from two different prompting results with the standard Reciprocal Rank Fusion (RRF) approach~\citep{cormack2009reciprocal}.
\zhuyun{TODO: put details about ensemble into Appendix. Add reranking experiments into appendix to justify the ensembling}.
% \inaim{Let's formally define $N$?}

Given the scores from LLMs (or after ensembling), we can now choose a new positive target: 
\begin{equation*}
\mathrm{positive}:  (q, P) \rightarrow (q, p_1 \in P)
    % positive: (q, p_{LLM-1st}) 
\end{equation*}
where $p_1$ is the highest scoring passage among $P$.
Importantly, $p_{1}$ can be different from $p_\text{seed}$ and conveys an approximation to the global preference of the LLM over the entire corpus.
% given the initial set of $P$.
\Cref{tab:fret_examples} lists examples where the $p_1$ differs from $p_\text{seed}$, demonstrating that the pair ($q, p_\text{seed}$) can be sub-optimal and there can be more relevant passages for $q$ globally.  

Similarly, the LLM scores can also be used to select hard negative passages as follows.
We assume that out of the $N$ nearest neighbor passages, the $k$ highest-scoring ones are at least more relevant than the rest.
% \jinhyuk{following equation is a bit strange. if we sample, use $\sim$.}\jrc{oops, I think I assumed we used all of them. I changed the equation.}
Hence, we sample hard negative passages from the rank between $k$ and $N$: 
%Assuming the top K passages ranked by the LLM are likely relevant, we sample hard negatives from those ranked after the K-th position:  
\begin{equation*}
\mathrm{negative}: (q, P) \rightarrow (q, p_{j} \sim P_{k + 1}^{N})
%  negative: (q, p_{LLM-kth}), k \in [K+1, N]
\end{equation*}
With our approach , we generate \dataset{} containing 6.6M examples, each of which containing a task, a query, a positive passage, and a negative passage.
% Table \ref{tab:fret_dataset} shows the statistic of \dataset{}.
% Implementation Details are in Appendix xxx.  

% \input{tables/fret-stats}


\subsection{Classification Data for Contrastive Learning}\label{sec:data_classificaiton}
While \citet{muennighoff2023mteb} shows a clear correlation between the model size and its classification performance (e.g., ST5~\citep{ni2022sentence} or SGPT~\citep{Muennighoff2022sgpt}), we claim that this behavior can be efficiently carved into a fixed-sized embedding model by directly training on the corresponding in-domain training sets.\footnote{We found that many classification tasks in MTEB~\citep{muennighoff2023mteb} are very application-specific, requiring specific granularity of representations.
For instance, MTEB contains Banking77~\citep{casanueva2020efficient}, which requires each text input to be classified into 77 distinct intents such as `card\_about\_to\_expire' or `card\_not\_working.'
At the same time, a review classification dataset such as IMDB~\citep{maas2011learning} requires only two labels, positive or negative.
We believe that such behaviors are better to be derived directly from the in-domain training sets whenever available.}
Specifically, we aim to seamlessly incorporate the MTEB classification training sets into our contrastive learning objective defined in \Cref{eq:contrastive} without any performance degradation on other tasks such as document retrieval.

% \jinhyuk{we might need to delete this given the ablation result}
Specifically, given a classification input text $x$ with a label $y \in \mathcal{Y}$, we pair each input $x$ with another input $x^+$, which shares the same label $y$, as a positive target.
At the same time, we randomly select a hard negative input $x^-$, whose label is from the remaining labels $\mathcal{Y}\setminus\{y\}$.
This approach is a simple version of the classification datasets pre-processed by \citet{su2022one}, but without using any model-specific embeddings.
However, during our experiments, we found that each $x^+$ might overlap with other positive example for a different mini-batch index, causing the false negative problem.
Hence, we assign a unique ID to each triple ($x$, $x^+$, $x^-$) and append the same unique ID to $x$, $x^+$, and $x^-$.
This effectively makes other distractors trivial but $x^-$ since the answers are always in the targets that share the same unique IDs with $x$ (i.e., $x^+$ and $x^-$).
% We found that this helps our models better calibrate the decision boundary for each classification task by putting more focus on $x^+$ and $x^-$.

\subsection{Additional Training Data}\label{sec:data_additional}
\paragraph{Pre-finetuning Data}
We use two pre-finetuning datasets.
First, we use the large-scale community QA dataset by \citet{Ni2021LargeDE}, which includes text pairs such question-answer from online forums and QA websites .
Additionally, we crawled title-body text pairs from the Web, which can be found from any websites as naturally occurring pairs.
Despite being very simple, recent works~\citep{wang2022text} showed that these naturally occurring text pairs are useful for pre-finetuning.

\paragraph{Fine-tuning Data}
In addition to \dataset{}, we use the following academic training datasets: Natural Questions~\citep{kwiatkowski2019natural}, HotpotQA~\citep{yang2018hotpotqa}, Fever~\citep{thorne2018fever}, MedMCQA~\citep{pal2022medmcqa}, SNLI~\citep{bowman2015large}, MNLI~\citep{williams2018broad}, and several in-domain classification training sets from MTEB~\citep{muennighoff2023mteb}.
For the multilingual model, we add training sets from MIRACL~\citep{zhang2023miracl}.
All datasets are pre-processed to have a unified encoding format (details in \Cref{sec:apdx_format}) for an input, a target, and a negative target.

==> sections/method.tex <==
\section{Method}

We train \ours{} based on a 1.5B language model \zhuyun{change to "1.5B pretrained Transformer language model"?} \zhuyun{1.5B or 1.2B?}.
We first pre-finetune \ours{} on a set of naturally occurring text pairs described in \Cref{sec:data_additional} following \citet{Ni2021LargeDE}.
We then further fine-tune \ours{} on a smaller set of fine-tuning datasets including \dataset{}, which also contain hard negatives.

\subsection{Pre-finetuning}
For smaller-scale dual encoders, it has been shown that training them with a large amount of unsupervised text pairs help improve the performance on various downstream tasks including document retrieval~\citep{lee2019latent,izacard2021contriever} and semantic similarity~\citep{gao2021simcse}.
Our goal of pre-finetuning is to expose a large amount of diverse text pairs, which seems necessary for smaller-scale text embedding models~\citep{wang2022text}.

\jinhyuk{this $N$ and $i$ is overlapping with $N$ and $i$ from section3. (they were written independently...)}
For a set of text pairs $\mathcal{D}_\text{pre} = \{(q_i, p_i)\}_{i=1}^N$ and a pre-trained language model $\mathcal{M}$ that outputs a sequence of token representations $\mathbb{R}^{n \times d}$ given $n$ input tokens, we obtain the vector representations of $q_i$ and $p_i$ as follows:
\begin{equation}\label{eq:text_rep}
\begin{split}
    \mathbf{q}_i &= \texttt{mean\_pool}[\mathcal{M}(t \oplus q_i)] \in \mathbb{R}^d \\
    \mathbf{p}_i &= \texttt{mean\_pool}[\mathcal{M}(p_i)] \in \mathbb{R}^d. \\
\end{split}
\end{equation}
Here, we prepend a dataset-specific task feature $t$ before each query, so each query is informed of which task is being optimized.
For pre-finetuning, we use either \textit{question answering} or \textit{search result} for the task feature $t$ depending on the dataset.
Then, for each mini-batch of size $B$, we optimize the contrastive learning objective with in-batch negatives:
\begin{equation}\label{eq:contrastive}
    \mathcal{L}_\text{pre} = \frac{1}{B}\sum_{i=1}^B \big[-\log \frac{e^{\text{sim}{(\mathbf{q}_i, \mathbf{p}_i})/\tau}}{\sum_{j=1}^B e^{\text{sim}(\mathbf{q}_i, \mathbf{p}_j)/\tau}}\big].
\end{equation}
In this work, we use the cosine similarity for the similarity function, $\text{sim}(\mathbf{x}, \mathbf{y}) = \frac{\mathbf{x}^\top\mathbf{y}}{||\mathbf{x}|| \cdot ||\mathbf{y}||}$, with a temperature parameter $\tau$.
Note that we do not utilize hard negatives during pre-finetuning and utilize the maximum batch size that fits into the device.
This found to be effective for document retrieval tasks as observed in previous work~\citep{wang2022text}.\jinhyuk{add more work}

\subsection{Fine-tuning}
For fine-tuning, we are given a set of $M$ fine-tuning datasets that are comprised of a dataset-specific task description, an input, a positive target, and a (hard) negative target: $[\mathcal{D}^{(1)}, \dots, \mathcal{D}^{(M)}]$ where $\mathcal{D}^{(m)} = \{(t^{(m)}, q_i, p_i^+, p_i^-)\}_{i=1}^N$.
We obtain the vector representations $\mathbf{q}_i$, $\mathbf{p}_i^+$, and $\mathbf{p}_i^-$ similar to \cref{eq:text_rep} where $t^{(m)}$ is used for the input: $\mathbf{q}_i = \texttt{mean\_pool}[\mathcal{M}(t^{(m)} \oplus q_i)]$.

For fine-tuning, we utilize the negative target $p_i^-$ as well as same tower negatives~\citep{moiseev2023samtone}, which adds $\{\mathbf{q}_j\}_{j=1}^B$ as additional negative targets except $j \neq i$.
Given a mini-batch of size $B$, we optimize the following objective:
\begin{equation}\label{eq:loss_main}
    \mathcal{L}_\text{main} = \frac{1}{B}\sum_{i=1}^B \big[-\log \frac{e^{\text{sim}(\mathbf{q}_i, \mathbf{p}_i^+)/\tau}}{\sum_{j=1}^B (e^{\text{sim}(\mathbf{q}_i, \mathbf{p}_j^+)/\tau} + \mathbbm{1}_{[j \neq i]}e^{\text{sim}(\mathbf{q}_i, \mathbf{q}_j)/\tau}) + e^{\text{sim}(\mathbf{q}_i, \mathbf{p}_i^-)/\tau}}\big].
\end{equation}
For the same tower negatives, we used the indicator variable $\mathbbm{1}_{[j\neq i]}$ to denote that we are iterating over $j$ except the current target index $i$.
Intuitively, the same tower negatives are helpful for the symmetric text embedding tasks such as measuring the semantic similarity of two sentences since $\{\mathbf{q}_j\}_{j=1}^B$ shares the same modality with $\mathbf{q}_i$ (e.g., query vs. query).
Finally, to support multiple different dimensions of embeddings, we add the MRL~\citep{kusupati2022matryoshka} loss, which optimizes \cref{eq:loss_main} with smaller sub-dimensions smaller than $d$.
% Later in our experiments, we show the effect of the same tower negatives for such symmetric tasks.

% \jinhyuk{describe bidrectionality if needed}
% \jinhyuk{mention mrl}

% \paragraph{Mini-Batch Sampling for Mixture}
% For classification, as described in \Cref{sec:data_classificaiton}, we append the same unique random string for each the input and the target so that ...
% \jinhyuk{describe more details on mixture rates, classification, }

==> tables/clf-test.tex <==
\begin{table}[t]
    \small
    \centering
	\caption{
	Learning classification (Class.) with \ours{}. We find that training with unique ids and same-label pairs help us integrate in-domain classification tasks better while maintaining the performance on retrieval tasks (BEIR).
	\jinhyuk{run experiments}
	}\label{tab:clf_test}
	\resizebox{0.40\linewidth}{!}{%
	\begin{tabular}{l|cc}
		\toprule
		& Class. & Retrieval \\
		\midrule
		Baseline (\dataset{} only) & & \\
		$+[1]$ In-domain datasets \\
		\quad\quad $+[2]$ Unique IDs \\
		\quad\quad $+[3]$ Label-based pairs \\
		
		\midrule
		$+[1, 2, 3]$ & \textbf{81.17} & \textbf{55.70} \\
        \bottomrule
	\end{tabular}
	}
\end{table}

==> tables/fret-stats.tex <==
\begin{table*}[t]
    \small
    \centering
    \begin{tabular}{l|r}
         \toprule 
         Task  & \# Queries \\ \midrule
         Question Answering & 3,057,845 \\
         Search & 2,634,064 \\
         Sentence Similarity & 574,331 \\
         Fact Checking & 330,246 \\
         \midrule
         Total & 6,596,486 \\
         \bottomrule
    \end{tabular}
    \caption{Distribution of the \textbf{F}ew-shot Prompted \textbf{Ret}rieval dataset (\dataset{}).
    \jinhyuk{more detail? or better be in a in-line table? (half column) \zhuyun{Statistics people maybe interested in:  1) passage lengths, 2) query lengths, 1)how often LLM-positive is not same as original passage. } Those sound great!}
    \mw{to me; I prefer not to release this stats; I think we should not talk about too much the stats of the generated data.}
    }
    \label{tab:fret_dataset}
\end{table*}

==> tables/label-test.tex <==
\eat{\begin{table}[t]
    \small
    \centering
	\caption{
	Do LLMs provide better labels for text retrieval datasets?
	We test different strategies of choosing positive and hard negative passages in \ours{} and MS-MARCO, and report their BEIR (nDCG@10) and STS (Spearman Correlation) performance. 
% 	\jinhyuk{run experiments; retriever score}
	\mw{Again, I think we can use less space for the ablation}
% 	\zhuyun{1) Perhaps we remove 5th and 10th. 2) Do we need GTR and XTR rows for this ablation? I only used 10 perecent msmarco so they won't be apple-to-apple}
	}\label{tab:label_test}
	\resizebox{0.50\linewidth}{!}{%
% 	\begin{tabular}{ll|cc}
% 		\toprule
% 		Positive & Hard Negative  & BEIR & STS \\ % & MS 
% 		\midrule
% 		\textit{MS-MARCO} \\
% 		\midrule
% 		Original passage (No pre-finetuning) & None & 41.79  & 77.52 \\ % & 33.33
% 		Original passage & None & 49.87 & \textbf{79.38} \\ %  & 35.98
% 		Original passage & RocketQA negatives~\citep{qu2021rocketqa} & 48.73 & 78.38 \\
% 		Original passage & Random nearest neighbor (10-200) & 50.31 & 78.17 \\ %  & 34.99
% 		Most relevant passage by LLM  & Random nearest neighbor (10-200) & 52.03 & 78.96 \\ %  & 38.62 
% 		Most relevant passage by LLM & 20th relevant passage by LLM & \textbf{52.29} & 78.96 \\ % & 37.04 
% % 		Original passage & RocketQA negatives \\
% % 		Original passage & RocketQA negatives (XTR-xxl by \citeauthor{lee2024rethinking}) & 52.29 & -  & \\
% 		\midrule
% 		\textit{\dataset{}} \\
% 		\midrule
% 		Original passage (No pre-finetuning) & None & 45.33 & 79.16 \\
% 		Original passage & None & 52.33 & 82.66 \\
% 		Original passage & Random nearest neighbor (10-200) & 51.37 & 82.00 \\
% 		Original passage & 20th relevant passage by Retriever & 51.96 & 82.26 \\
% 		Original passage & 2nd relevant passage by LLM  & 50.47 & 81.63 \\
% % 		Original passage & 5th relevant passage by LLM  & 51.18 & 81.87 \\
% 		Original passage & 10th relevant passage by LLM  & 51.71 & 82.20 \\
% 		Original passage & 20th relevant passage by LLM  & 52.51 & 82.59 \\

% 		Most relevant passage by LLM & None & 53.07 & 82.88 \\
% 		Most relevant passage by LLM & Random nearest neighbor (10-200) & 52.60 & 82.85 \\
% 		Most relevant passage by LLM & 2nd relevant passage by LLM & 50.36 & 82.56 \\
% % 		Most relevant passage by LLM & 5th relevant passage by LLM & 52.65 & 82.63 \\
% 		Most relevant passage by LLM & 10th relevant passage by LLM & 53.06 & 82.96 \\
% 		Most relevant passage by LLM & 20th relevant passage by LLM & \textbf{53.39} & \textbf{83.14} \\
% % 		Most relevant passage by LLM & 20th relevant passage by Retriever &  \\
%         \bottomrule
% 	\end{tabular}
	
	\begin{tabular}{ll|cc}
		\toprule
		Positive ($p^+$) & Hard Negative ($p^-$) & BEIR & STS \\ % & MS 
		\midrule
		\multicolumn{4}{l}{\textit{MS-MARCO}} \\
		\midrule
		$p_\text{seed}$ (w/o pre-finetuning) & None & 41.79  & 77.52 \\ % & 33.33
		$p_\text{seed}$ & None & 49.87 & \textbf{79.38} \\ %  & 35.98
% 		$p_\text{seed}$ & Negatives by~\citet{qu2021rocketqa} & 48.73 & 78.38 \\
		$p_\text{seed}$ & $p \sim P_1^N$ & 50.31 & 78.17 \\ %  & 34.99
		$p_1$ & $p \sim P_1^N$ & 52.03 & 78.96 \\ %  & 38.62 
		$p_1$ & $p_{20}$ & \textbf{52.29} & 78.96 \\ % & 37.04 
% 		Original passage & RocketQA negatives \\
% 		Original passage & RocketQA negatives (XTR-xxl by \citeauthor{lee2024rethinking}) & 52.29 & -  & \\
		\midrule
		\textit{\dataset{}} \\
		\midrule
		$p_\text{seed}$ (w/o pre-finetuning) & None & 45.33 & 79.16 \\
		$p_\text{seed}$ & None & 52.33 & 82.66 \\
		$p_\text{seed}$ & $p \sim P_1^N$ & 51.37 & 82.00 \\
		$p_\text{seed}$ & $p_{20}$ by retriever & 51.96 & 82.26 \\
		$p_\text{seed}$ & $p_{2}$ & 50.47 & 81.63 \\
% 		$p_\text{seed}$ & 5th relevant passage by LLM  & 51.18 & 81.87 \\
		$p_\text{seed}$ & $p_{10}$ & 51.71 & 82.20 \\
		$p_\text{seed}$ & $p_{20}$ & 52.51 & 82.59 \\

		$p_1$ & None & 53.07 & 82.88 \\
		$p_1$ & $p \sim P_1^N$ & 52.60 & 82.85 \\
		$p_1$ & $p_{2}$ & 50.36 & 82.56 \\
% 		Most relevant passage by LLM & 5th relevant passage by LLM & 52.65 & 82.63 \\
		$p_1$ & $p_{10}$ & 53.06 & 82.96 \\
		$p_1$ & $p_{20}$ & \textbf{53.39} & \textbf{83.14} \\
        \bottomrule
	\end{tabular}
	}
\end{table}
}

\begin{table}[t]
    \small
    \centering
	\caption{
	Do LLMs provide better labels for text retrieval datasets?
	We test different strategies of choosing positive and hard negative passages in \ours{} and MS-MARCO, and report their BEIR (nDCG@10) and STS (Spearman Correlation) performance. 
% 	\jinhyuk{run experiments; retriever score}
% 	\mw{Again, I think we can use less space for the ablation}
% 	\zhuyun{1) Perhaps we remove 5th and 10th. 2) Do we need GTR and XTR rows for this ablation? I only used 10 perecent msmarco so they won't be apple-to-apple}
	}\label{tab:label_test}
	\resizebox{0.55\linewidth}{!}{%
	\begin{tabular}{ll|cc}
		\toprule
		Positive ($p^+$) & Hard Negative ($p^-$) & BEIR & STS \\ % & MS 
		\midrule
		\multicolumn{4}{l}{\textit{MS-MARCO}} \\
		\midrule
		%$p_\text{seed}$ (w/o pre-finetuning) & None & 41.79  & 77.52 \\ % & 33.33
		$p_\text{seed}$ & None & 49.87 & \textbf{79.38} \\ %  & 35.98
% 		$p_\text{seed}$ & Negatives by~\citet{qu2021rocketqa} & 48.73 & 78.38 \\
		$p_\text{seed}$ & $p \sim P \setminus \{p_\text{seed}\}$ & 50.31 & 78.17 \\ %  & 34.99
		$p_1$ & $p \sim P \setminus \{p_1\}$ & 52.03 & 78.96 \\ %  & 38.62 
		$p_1$ & $p_{20}$ & \textbf{52.29} & 78.96 \\ % & 37.04 
% 		Original passage & RocketQA negatives \\
% 		Original passage & RocketQA negatives (XTR-xxl by \citeauthor{lee2024rethinking}) & 52.29 & -  & \\
		\midrule
		\textit{\dataset{}} \\
		\midrule
		%$p_\text{seed}$ (w/o pre-finetuning) & None & 45.33 & 79.16 \\
		$p_\text{seed}$ & None & 52.33 & 82.66 \\
		$p_\text{seed}$ & $p \sim P \setminus \{p_\text{seed}\}$ & 51.37 & 82.00 \\
		$p_\text{seed}$ & $p_{20}$ & 51.96 & 82.26 \\
		%$p_\text{seed}$ & $p_{2}$ & 50.47 & 81.63 \\
% 		$p_\text{seed}$ & 5th relevant passage by LLM  & 51.18 & 81.87 \\
		%$p_\text{seed}$ & $p_{10}$ & 51.71 & 82.20 \\
		%$p_\text{seed}$ & $p_{20}$ & 52.51 & 82.59 \\

		$p_1$ & None & 53.07 & 82.88 \\
		$p_1$ & $p \sim P \setminus \{p_1\}$ & 52.60 & 82.85 \\
%		$p_1$ & $p_{2}$ & 50.36 & 82.56 \\
% 		Most relevant passage by LLM & 5th relevant passage by LLM & 52.65 & 82.63 \\
		%$p_1$ & $p_{10}$ & 53.06 & 82.96 \\
		$p_1$ & $p_{20}$ & \textbf{53.39} & \textbf{83.14} \\
        \bottomrule
	\end{tabular}
	}
\end{table}

==> tables/sts-clf-test.tex <==
\begin{table}[t]
    \small
    \centering
	\caption{
	Learning semantic similarity (left) and classification (right) with \ours{}.
	For semantic similarity, we test the symmetric formatting (Sym.) and the same tower negatives (SamToNe) with different mixture rates for \dataset{}-sentence-similarity ($\alpha_\text{sent}$) and NLI datasets ($\alpha_\text{nli}$).
	For classification, we test prepending unique identifiers (IDs) and using label-based pairs (Pair) with a different mixture rate for the classification datasets ($\alpha_\text{class.}$).
	\jinhyuk{unmixed batch exp}
	\mw{do we need this?}
	}\label{tab:sts_clf_test}
	\resizebox{0.42\linewidth}{!}{%
	\begin{tabular}{cccc|cc}
		\toprule
		$\alpha_\text{sent}$ & $\alpha_\text{nli}$ & Sym. & SamToNe & STS & Retrieval \\
		\midrule
		0.0 & 0.0 & - & - & 80.63 & \textbf{53.54} \\
% 		0.0 & 1.0 & - & - & 82.59 & 53.29 \\
% 		1.0 & 0.0 & - & - & 79.86 & 53.53 \\
		1.0 & 1.0 & - & - & 81.21 & 53.37 \\
		\midrule
% 		0.0 & 1.0 & - & \checkmark \\
% 		0.0 & 1.0 & \checkmark & - \\
% 		0.0 & 1.0 & \checkmark & \checkmark \\
% 		\midrule
% 		1.0 & 0.0 & - & \checkmark \\
% 		1.0 & 0.0 & \checkmark & - \\
% 		1.0 & 0.0 & \checkmark & \checkmark \\
% 		\midrule
		1.0 & 1.0 & - & \checkmark & 83.06 & 52.97 \\
		1.0 & 1.0 & \checkmark & - & 84.39 & 53.13 \\
		1.0 & 1.0 & \checkmark & \checkmark & 84.46 & 52.93 \\
		\midrule
		1.0 & 0.0 & \checkmark & \checkmark & 83.14 & 53.16 \\
		0.0 & 1.0 & \checkmark & \checkmark & \textbf{84.62} & 52.93 \\
		\midrule
		1.0 & 2.0 & \checkmark & \checkmark & 84.52 & 52.91 \\
		2.0 & 1.0 & \checkmark & \checkmark & 84.28 & 52.95 \\
        \bottomrule
	\end{tabular}
	}\quad\quad
	\resizebox{0.32\linewidth}{!}{%
	\begin{tabular}{ccc|cc}
		\toprule
		$\alpha_\text{class.}$ & IDs & Pair & Class. & Retrieval \\
		\midrule
		0.0 & - & - & 70.26 & \textbf{53.16} \\
		1.0 & - & - & \textbf{80.99} & 52.83 \\
		\midrule
		1.0 & - & \checkmark & 78.49 & 52.56 \\
		1.0 & \checkmark & - & 77.77 & 52.92 \\
		1.0 & \checkmark & \checkmark & 79.19 & 52.99 \\
		\midrule
		2.0 & \checkmark & - & 78.27 & 53.13 \\
		4.0 & \checkmark & - & 78.61 & 52.85 \\
		\midrule
		2.0 & \checkmark & \checkmark & 79.78 & 52.98 \\
		4.0 & \checkmark & \checkmark & 79.99 & 52.63 \\
        \bottomrule
	\end{tabular}
	}
\end{table}
